Global parameters of Quasars with anomalous electromagnetic spectrum

The thesis concerns the analysis of the Active Galactic Nuclei. These are galaxies with an active core. The most luminous type of Active Galactic Nuclei is Quasar. It contains the supermassive black hole at the center. One of the least known subtype of Quasars are: Weak emission-Line Quasars. Their recognizable feature are weak emission-lines. The primary goal of PhD thesis is to evaluate the global parameters such as: the black hole mass, the accretion rate, spin of the black hole, and the inclination of weak emission-line quasars based on the continuum fit method. This method apart from the literature black hole masses estimation methods does not depend on the observed Full Width at Half Maximum of emission line, which could be biased due to the weakness or lack of the emission lines in these quasars. Using the Spectral Energy Distribution of quasars, I have fitted the geometrically thin and optically thick accretion disk model described by Novikov \& Thorne equations. I have obtained the model of the continuum of the accretion disk for the 10 weak emission-line quasars. The second project concerned the description of abnormal, deep absorption of SDSS J110511.15+530806.5 quasar. I checked the correctness of the thesis posed that corona and warm skin concept above/around an accretion disk explain this phenomenon.

==> acronym.tex <==
\newacronym{AGN}{AGN}{active galactic nucleus}
\newacronym{AD}{AD}{accretion disk}
\newacronym{WLQ}{WLQ}{weak emission-line quasar}
\newacronym{BH}{BH}{black hole}
\newacronym{SMBH}{SMBH}{Suppermassive black hole}
\newacronym{QSO}{QSO}{quasar}
\newacronym{BLR}{BLR}{Broad Line Region}
\newacronym{NLR}{NLR}{narrow Line Region}
\newacronym{UV}{UV}{ultraviolet}
\newacronym{IR}{IR}{infrared}
\newacronym{SF}{SF}{starformation}
\newacronym{IGM}{IGM}{intergalactic medium}
\newacronym{EW}{EW}{Equivalent Width}
\newacronym{FWHM}{FWHM}{Full Width at Half Maximum}
\newacronym{SED}{SED }{Spectral Energy Distribution}
\newacronym{NT}{NT}{Novikov-Thorne}
\newacronym{SS}{SS}{Shakura-Sunayaev}


% \section*{Abbreviations}

% class `abbrev': abbreviations:
% \newacronym{agn}{AGN}{Active galactic nucleus}
% \newacronym{agns}{AGNs}{Active galactic nuclei}
% \newacronym{AD}{AD}{Accretion disk}
% \newacronym{WLQ}{WLQ}{Weak emission-line quasar}
% \newacronym{WLQs}{WLQs}{Weak emission-line quasars}
% \newacronym{BH}{BH}{Black hole}
% \newacronym{BHs}{BHs}{Black holes}
% \newacronym{SMBH}{SMBH}{Suppermassibe black hole}
% \newacronym{QSO}{QSO}{Quasar}
% \newacronym{QSOs}{QSOs}{Quasars}
% \newacronym{BLR}{BLR}{Broad Line Region}
% \newacronym{NLR}{NLR}{Narrow Line Region}
% \newacronym{UV}{UV}{Ultraviolet}
% \newacronym{SF}{SF}{Starformation}
% \newacronym{IGM}{IGM}{intergalactic medium}
% \newacronym{EW}{EW}{Equivalent Width}
% \newacronym{FWHM}{FWHM}{Full Width at Half Maximum}
% \newacronym{SED}{SED }{Spectral Energy Distribution}
% \newacronym{NT}{NT}{Novikov-Thorne}
% \newacronym{SS}{SS}{Shakura-Sunayaev}



==> ch8.tex <==
% \chapter{Discussion}

% \section{Calculations for the Potential Absorption Source}\label{sec:calc_abs}
% The origin of such abnormal deep absorption in the J1105 is interesting. In this paragraph, I have focused on two possible scenarios for the origin of the absorber. I have calculated two of the most plausible explanations.
% % \CIV\ is discussed in the \cite{Stone_abs_2019} work. The Figure 3 of their paper represents the velocity distribution of \CIV\ absorption. Regarding the redshift which is calculated, I have ruled out the low-velocity intrinsic absorber which reached $\beta = V/c = 0.02$. The more plausible explanation either the high-velocity absorber or intervening system reach the maximum of $\beta = 0.10$.
% % The minimum of the Gauss for J1105 is at $\nu_{abs} = 1.99526 \times 10^{15}$ Hz, so the $\lambda_{abs}$ is on 1502 \AA\ (rest frame).
% In Fig. \ref{fig:4_gaussians} I have presented the two Gaussian function descriptions. The values of each of them were converted from the XSPEC fitting to wavelength in rest frame interpretation. The Gaussian function observed in the rest frame at 1516 \AA\ is the one that dominates the fit. However, all two of them are needed for the goodness of fit. 

% %1516 \AA\ (in rest frame = $2.792\times10^{-3}$ keV in observed frame)
% \begin{figure}[H]
%   \centering
%     \includegraphics[width=1.0\textwidth]{figures/corona/gaussians_new_v3.png}
%  \caption{The illustration of the two Gaussian's}{The illustration of the two Gaussian's, with $\sigma = 332$ \AA, EW = 714 \AA; $\sigma = 375$ \AA, EW = 124 \AA.}
%  \label{fig:4_gaussians}
% \end{figure}
% % $\sigma = 75$ \AA, EW = 1.88 \AA; $\sigma = 10$ \AA, EW = 0.125 \AA.

% \begin{table}[ht]
%     \centering
%     \caption{Conversion of energies in the observed frame to the rest frame.}{Comparison of the observed frame energies and sigmas (keV) establish from the fitting of Gaussian functions with converted wavelength to the rest frame in \AA.}
%     \begin{tabular}{c|c|c|c}
%      & & observed frame (keV) & rest frame (\AA) \\
%     \hline
%     \multirow{2}{*}{First Gaussian} & Line E & $(2.792 \pm 0.015) \times 10^{-3}$&  $1516\pm10$\\
%     \cline{2-4}
%     &$\sigma$ & $(5.842\pm 0.069) \times 10^{-4}$ & $332\pm69$ \\
%     \cline{2-4}
    
%     \hline
%     \multirow{2}{*}{Second Gaussian} & Line E & $(2.125\pm0.022)\times 10^{-3}$ & $1992\pm20$ \\
%     \cline{2-4}
%     & $\sigma$ & $(3.874 \pm 0.117)\times 10^{-4}$ &  $375\pm 64$ \\
%     \cline{2-4}
%     \hline
%     \end{tabular}
    
%     \label{tab:observed_energy_rest_wave}
% \end{table}


% \subsection{How far from the galaxy is the absorption cloud? }

% The minima of the Gauss functions (Fig. \ref{fig:4_gaussians}) for J1105 in the rest frame are at $1516\pm10$ \AA, $1992\pm20$ \AA\ with $\sigma$ $332\pm69$ and $375\pm 64$ receptively.
% %$380\pm 64$ receptively (rest frame).
% If we assume that the global absorption in J1105 is caused by an extended cloud that absorbs \MgII\ (2796 \AA, 2803 \AA), then from equation $z = \frac{\lambda_{obs}}{\lambda_{em}} - 1 = \frac{\lambda_{abs}}{2800 \small\angstrom} - 1$ we are able to establish its $z_{1, \mathrm{MgII}} = - 0.4585$, $z_{2, \mathrm{MgII}} = - 0.2885$,  This is the distance of this cloud/absorber from the host galaxy. However, if we assume that the cloud absorbs \CIV\ (1548 \AA, 1551 \AA), then its $z_{1, \mathrm{CIV}} = - 0.0213$, $z_{2, \mathrm{CIV}} = + 0.2859$.
% %$z_3 = - 0.2889$, $z_4 = - 0.1707$.
% %$z_3 = + 0.2853$, $z_4 = + 0.4990$.

% % The redshift of the cloud/clouds/absorber might be at $z_1 = -0.46$ or $z_2 = -0.03$ from the QSO, if we assume \MgII\ or \CIV\ medium respectively.

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=0.8\textwidth]{figures/corona/clouds_MgII.jpg}
%  \caption{A scheme of potential absorption \MgII\ clouds in front of the quasar}
%   \label{fig:MgII_clouds}
% \end{figure}

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=0.8\textwidth]{figures/corona/clouds_CIV.jpg}
%  \caption{A scheme of potential absorption \CIV\ clouds}
%  \label{fig:CIV_clouds}
% \end{figure}

% \subsection{If We Assume the Wind is the Absorber}

% % The second case might be the wind not a cloud which causes the broad absorption.
% % An interesting specification of the quasar with strong absorption lines one can find in \cite{Stone_abs_2019} work.
% An absorption line in the spectrum of a NAL or BAL quasar is redshifted or blueshifted according to its lab position. Assuming the shift is caused by the Doppler effect and the absorber is a large-scale outflow, we can estimate the velocity of the absorbing material.

% % Redshift of the order 0.03 indicates that fast wind may be the cause of an absorption in this case not the IGM.

% % I have assumed that the velocity of the wind can be calculated using the Doppler dependency for the light.

% \begin{equation}
%     \nu_{obs} = \nu_{em} \sqrt{\frac{1-\beta}{1+\beta}},
% \end{equation}
% \noindent  where $\beta = \frac{V}{c}$ and $V$ is velocity of a wind,
% \noindent  then after rearrangement:
% \begin{equation}
%     \lambda_{em} = \lambda_{abs} \sqrt{\frac{1-\beta}{1+\beta}} = > \frac{1-\beta}{1+\beta} = \left(\frac{\lambda_{em}}{\lambda_{abs}}\right)^2
% \end{equation}
% \noindent From definition of redshift we know that $\lambda_{obs} = \lambda_{em} (1+z)$\\
% \noindent therefore:
% \begin{equation}
%     \frac{1-\beta}{1+\beta} = \frac{1}{(1+z)^2} => (1-\beta)(1+z)^2 = (1+\beta)
% \end{equation}
% \begin{equation}
%     (1+z)^2 - 1 = \beta (1+(1+z)^2)
% \end{equation}
% \noindent and final equation for $\beta$ looks like:
% \begin{equation}
%     \beta = \frac{(1+z)^2-1}{(1+z)^2+1}
% \end{equation}

% \noindent The final parameters for this section look like:
% % \begin{itemize}[noitemsep,topsep=0pt]
% %   \item for z = 0.03; $\beta$ = 0.0295 and V = -8860 \kms, 
% %   \item for z = 0.46; $\beta$ = 0.3613 and V = - 108330 \kms. 
% %   \item for z = (?); $\beta$ = (?) and V = (?) \kms, 
% %   \item for z = (?); $\beta$ = (?) and V = (?) \kms. 
% % \end{itemize}
% \begin{table}[ht]
%     \centering
%     \begin{tabular}{c|c|c|c}
%         & redshift & $\beta$ & V (km/s) \\
%         \hline
%         \multirow{2}{*}{Mg II}
%           & $-0.4585^{+0.0031}_{-0.0033}$ & $-0.3605^{+0.0018}_{-0.0021}$  & $-108135^{+555}_{-615}$  \\
%           & $-0.2885\pm 0.0071$ & $-0.2482^{+0.0051}_{-0.0053}$ & $-74447^{+1543}_{-1577}$ \\
%           \hline
%         \multirow{2}{*}{CIV}
%         & $-0.0213\pm0.0058$ & $-0.0211^{+0.0055}_{-0.0057}$  & $-6330^{+1698}_{-1710}$  \\
%           & $+0.2859\pm 0.0013$ & $0.2463^{+0.0094}_{-0.0096}$ & $73887^{+2827}_{-2871}$ \\
%     \end{tabular}
%     \caption{The parameters of winds of \MgII\ and \CIV}
%     \label{tab:redshift_beta_velocityl}
% \end{table}

% \noindent The negative velocity indicates that the wind is blowing in our direction. 

% \cite{Stone_abs_2019} classified the Quasar absorption lines systems in view of their velocity distribution. Structures within $ V \leq$ 3000 \kms\ are called associated absorption lines. Systems with velocity separation 3000 - 12 000 \kms\ are dominated by intrinsicality or outflows from the QSO. Systems with velocity $\geq$ 12 000 \kms\ are disconnected from the QSO (see reference therein).

% According to \cite{Stone_abs_2019}, our first case (i.e. \MgII\ absorption clouds) points out the intervening system. In the second case, the outflow is the first Gaussian.

 
% %pointed out that if one assumes that the Quasar absorption lines systems are a constraint on the broad velocity, one can find the origin of the lines. They
% % a) pozycji: 1450 Angstromów; EW = 714 Angst.
% % b) 1992; EW = 124 Angst.
% % c) 1991; EW = 1.88 Angst.
% % d) 2322; EW = 0.125 Angst.

% \subsection{The column density of J1105}\label{sec:NH}
% In this subsection, I have estimated the ion column densities, $N$, of the absorbers. Recent results of \cite{Saez2021_NH} about wind properties in PG 2112+059 was taken into account. Equation (9), (10), and (12) in \cite{Saez2021_NH} indicated the relation of EW and $N_j$ for the single Gaussian. However, in the case of J1105, I have to use two doublets of absorption, namely the \CIV\ and \MgII\ lines.
% Using their Equation (12) for line doublet I was able to calculate $N_j$ of each Gaussian function in the optically thin regime for a fixed value of the ionization parameter and metallicity. 

% \begin{equation}
%     N_j \approx \frac{m_e c^2}{\pi e^2 (f_b \lambda^2_b+f_r \lambda^2_r)} EW,
% \end{equation}
% \noindent where b and r stands for parameters of the blue and red doublet respectively. $f$ is an oscillator strengths taken from \cite{Griesmann2000Carbon, Morton2003Magnesium}. The results are presented in the Tab. \ref{tab:NH_J1105}.


% \begin{table}[ht]
%     \centering
%     \begin{tabular}{c|c|c|c}
%     & & log$(N_j)$ & log$(N_j)$\\
%     & EW(\AA)$^*$ & \CIV ($cm^{-2}$) & \MgII ($cm^{-2}$) \\
%     \hline
%     First Gaussian & $714^{+145}_{-147}$  & $17.027^{+0.080}_{-0.010}$ & $16.003^{+0.080}_{-0.010}$ \\
%     Second Gaussian & $124^{+20}_{-21}$ & $16.266^{+0.065}_{-0.080}$ & $15.242^{+0.065}_{-0.080}$ \\
% %        & 14.447 & 13.423 & 1.88  \\
% %& log$(N_j)$
%     \end{tabular}
%     \caption{The column density of J1105}
%     \begin{quote}
%         * EW in rest frame
%     \end{quote}
%     \label{tab:NH_J1105}
% \end{table}

% The column densities of J1105 are in the range of previous researches about absorption in QSOs. For instance, \cite{Dobrzycki2007} established the mean ion column densities of CIV is $15.265\pm0.135$ for mini-BAL system. They have determined the ion column densities of the individual components in HS1603+3820 quasar e.g. \MgII\ of system B is $15.106\pm0.155$. The total N of ion \CIV\ varies from $13.200\pm0.035$ to  $15.471\pm0.085$.
% %They identified intervening systems at$z_{abs}$ 1.9266 and 2.2622

% Moreover, \cite{Saez2021_NH} indicate that the logarithmic values of column densities of CIV in BAL QSO PG 2112+059 vary during 13 years from 15.38 to 15.81. If they assumed the covering factor $\sim$ 60 then log $N_{CIV}$ = 16.12.


% %or even 16.12 for the covering factor of 60 \%.

% %Wind min -10595/-6317 - max -27129/-23336
% %Mg z 2.477 $12.123\pm0.300$ or $11.915\pm0.416$ or $12.903\pm0.115$ or 13.027/13.014
% %The total N of ion Mg II $15.106 \pm 0.155$ at $z_{abs}$ 2.48
% %$15.270\pm0.105$ for $z_{abs}$ 2.44,  for $z_{abs}$ 2.55 CIV $15.272\pm0.967$
% %or $15.200\pm1.134$ for $z_{abs}$ 2.55
% \section{Discussion}

% In Fig. \ref{fig:AD_corona_vicinity} I present the potential idea of an accretion disk and warm skin concept, which might be seen in J1105. \cite{Czerny2003corona_highacc} represent the concept of the bright AGN with a warm skin above the AD. A similar concept of warm skin, which wraps around the inner part of AD is presented here.
% \begin{figure}[H]
%   \centering
%     \includegraphics[width=0.8\textwidth]{figures/corona/warm_skin_J1105.jpg}
%  \caption{The vicinity of the J1105}{My view how the vicinity of the J1105 might look like}
%  \label{fig:AD_corona_vicinity}
% \end{figure}

% The AGNSED is a more sophisticated code with the same approach as QSOSED, but with all the free parameters presented in Tab. \ref{tab:agnsed_fitting_parameters}. However, as a first order approach, the warm skins from \cite{Czerny2003corona_highacc, MN_BCZ_skin2004} and \cite{KubotaDone_2018} model, look good enough to examine the nature of J1105.

% Primary I have fitted the QSOSED model with two Gaussian functions. The first Gaussian is the most dominant. The second seems to be crucial. The QSOSED model assumes the fixed parameters of the corona, the warm skin, and the disk size. I have chosen the AGNSED model with free parameters to get to know J1105 nature better. Moreover, I tried to find the best $kT_{e,hot}$ parameters. In this case, I have also tried many variants. It turned out that the best value is fixed to 100 keV, same as \cite{KubotaDone_2018} approach.
% I was able to make an even better fit procedure and obtained the reduced $\chi^2$ from \textbf{2.80} to: \textbf{2.056}. Not much improvement regarding the global parameters of the objects was observed.
% In the first order of approximation of the modeling procedure, I have fitted only one Gaussian function, the reduced $\chi^2$ was 7.0912. It seems that this object in particular needed more functions that described the absorption. Another Gaussian's were needed. However, when I have tried to narrow the Gaussian's down I obtained a not well fitted model. The reduced $\chi^2$ of the worse fit was > 10. 
% %To do that I added the third and the fourth Gaussian functions respectively.

% Besides the improved value of the reduced $\chi^2$, one of the most crucial take away is that \textbf{the AGNSED provide a better understanding of the physics and boundaries of the corona, the warm skin, and the disk size}. The mentioned parameters are within the assumptions of \cite{Czerny2003corona_highacc} and \cite{KubotaDone_2018} approaches (for more details please see their Table 1 and  Table 2 respectively).

% Unfortunately, \cite{Czerny2003corona_highacc} and \cite{KubotaDone_2018} objects do not contain such massive SMBH as J1105. In their studies, the \mbh\ is $10^8\mMsun$. However, the physics and corona/warm skin/disk description should not vary very much. Below I would like to compare parameters from three different studies.

% I would like to remind the \dotm\ of J1105 is equal to $0.274 \pm 0.001$. 
% The corona/warm skin concept of Mrk 359 by \cite{Czerny2003corona_highacc} indicate the \dotm = 0.3. Additionally, \cite{KubotaDone_2018} studied three close by objects ($z<0.16$). One of them PG 1115+407 has similar accretion rate $\sim$ 0.4.

% Moreover the $\Gamma_{warm}$ = $2.722\pm0.153$ of J1105 is similar to one obtained for PG 1115+407; $\Gamma_{warm}$ = 3.06 and Mrk 359 with $\Gamma_{warm}$ = 3.32. 

% % Moreover, the $\Gamma_{warm}$ = $2.722\pm0.153$ for \textbf{AGNSED} is within an error range of fixed value 2.5 in \textbf{QSOSED} study.

% % above the cold and optically thick disk of a temperature 0.2-0.5 keV, there is a warm layer with a temperature
% % of 1.0-1.5 keV and an optical depth around 10.

% Comparing study with QSOSED vs AGNSED as a main component of modeling, I have found that the $kT_{e, warm}$ = $0.356^{+4.876}_{-0.350}$ (keV) is a better description than the fixed value of 0.2 keV. I support this statement with the fact that the $kT_{e, warm}$ of \cite{KubotaDone_2018} study has 0.50 keV. Unfortunately, some errors are in the range of 1 $\sigma$ (or above). However, neither \cite{Czerny2003corona_highacc} nor \cite{KubotaDone_2018} included errors. Regarding the corona/warm skin size, J1105 has $R_{hot}$ = $58.54\pm3.36$ $r_g$  and $R_{warm}$  = $430.0^{+50.0}_{-11.0}$ $r_g$, comparing to $R_{warm}$ of Mrk 359 = $300 R_{Schw}$ ($R_{Schw} \sim 2 r_g$). The difference may be caused due to the divergence between \mbh. Nevertheless, the description of the corona/warm skin for J1105 is well established and comparable with literature studies.

% Contrary to the massive black holes, \cite{Zhang2000warmskin} modeled sources GRS 1915+105 and GRO J1655-40. Their study revealed a three-layered atmospheric structure in the inner region of AD. They found out a warm skin with T = 1.0-1.5 keV and an optical depth $\sim$ 10. They sum up the temperatures of the cold disk of $\sim 10^6K$, the warm skin $\sim 10^7K$, and corona $\sim 10^9K$ indicated the complicated phenomena around such objects (i.e. corona/warm skin explanation). However, they focused on the AD of the stellar mass black holes. GRO J1655-40 - has a black hole $\sim 7$ \Msun, GRS 1915+105 - $\sim 12 $ \Msun. In their Figure 2, one can see that the concept of the corona is very extensive. However, due to the very large \mbh\ difference, it should not be against the J1105 nature explanation, quite the contrary. 

% \cite{Meusinger2016} study of J1105 indicated that it has reddening steeper than in the Small Magellanic Cloud, perhaps even steeper than for IRAS 14026+4341 galaxy. They could not either find a good reddening/extinction solution for the case of J1105. They classify it as a strongly reddened narrow-line quasar. \cite{Jiang_2013} argued that such an unusual reddening law is based on a speculative assumption of an exotic dust grain size distribution that lacks large grains.

% Using \cite{Weymann1979} approach, \cite{Stone_abs_2019} distinguish three components of the velocity distribution of NALs: the uniform distribution of very high velocity components which is unassociated with the QSO; the influence of the virialized material clustered around the QSO itself, or associated with material ejected from the QSO. Regarding the values from Sec. \ref{sec:calc_abs}, the plausible explanation of the origin of the absorption in J1105 is \textbf{ the strong outflow represented by the first Gaussian function} and \textbf{the intervening material} e.g. dwarf galaxy \textbf{along the line of sight} seen as the second Gaussian curve in the spectrum. Nevertheless, the intervening material may explain both Gaussian functions. Regarding my results, I cannot exclude either NAL or BAL phenomena as an explanation of the nature of J1105.
% However, such wide absorption has not been observed in the sources of BALs. Further investigation was needed. The explanation of the abnormal properties of J1105 might lay at the root of the warm skin concept.

% My result indicated that the deep absorption in J1105 could be explained by two Gaussian functions which may describe two different clouds. The \CIV\ as an absorbing material is more plausible due to the fact that $\lambda_{min}$ of the main Gaussian is 1516 \AA\, whereas the laboratory line of \CIV\ lies at 1548\AA\ and 1551 \AA. The clouds or even a wind contains mostly \CIV\ which absorbs radiation from an AD/corona of the J1105. The most dominant Gaussian with $\sigma = 375$ \AA\ has a strength of nearly 90\% of the whole recess. Regarding the redshifts of the potential clouds, one can see that for \MgII\ case two clouds along the line of sight of observer occurred. Surprisingly in the \CIV\ case (Fig. \ref{fig:CIV_clouds}) one of the clouds is 'behind' the J1105! It seems that it is the wind component or Failed Radiatively Accelerated Dusty Outflow (FRADO) observed by Czerny's group. This wind falls to the AD. 

% The column density of ions for J1105 excluded either mini-BAL or BAL as an explanation of the deep absorption. Neither of the values of $N_j$ explains such an abnormal feature. Either column density of ions \CIV\ or \MgII\ of \cite{Dobrzycki2007} investigation or recently done by \cite{Saez2021_NH} regarding \CIV\ ion.

% In summary of the nature of the SDSSJ110511.15+530806.5 quasar I have presented two visual explanation of this phenomena (Fig. \ref{fig:J1105_wind}, Fig. \ref{fig:J1105_2galaxies}).

% This chapter will be concluded as a paper soon. I have found more objects with very high \mbh\ and abnormal features with their spectra. This work is in progress and I will examine it further.
% % AGNSED - It takes into account the influence of AD, corona, and warm skin.

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=0.65\textwidth]{figures/corona/winds-24.jpg}
%  \caption{An explanation of the nature of J1105 - winds.}
%  \label{fig:J1105_wind}
% \end{figure}

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=0.65\textwidth]{figures/corona/2galaxies-25.jpg}
%  \caption{An explanation of the nature of J1105 - two dwarf galaxies.}
%  \label{fig:J1105_2galaxies}
% \end{figure}

% % $\Gamma_{warm}$ = 3.06 which is similar to $\Gamma_{warm}$ & $2.722 \pm 0.153$ of J1105.  $\Gamma_{warm}$ = 3.32 for Mrk 359

% % $r_{skin}$ 300 in Rsch,
% % $\tau_{skin}$,
% % Tskin 3 keV, 
% % tau of warm absorber 0.25,
% % f of warm absorber 0.5,
% % z min 100, z max 10 000 rsch

% %   &  \dotm & $0.274 \pm 0.001$\\
% %         & cos \incl & $0.841 \pm 0.003$ \\
% %       & $a_*$ & $0.36 \pm 0.02$ \\
% %     & $kT_{e, hot}$ ( keV) & 100 (fixed)* \\
% %     & $\Gamma_{hot}$ & $1.300^{+1.545}_{-1.300}$ \\
% %      & $R_{hot}$ ($r_g$) &  $58.54 \pm  3.36$ \\
    
% %       & $kT_{e, warm}$ ( keV) & $0.356^{+4.876}_{-0.350}$ \\
% %              & $\Gamma_{warm}$ & $2.722 \pm 0.153$ \\
% %               & $R_{warm}$ ($r_g$) & $430.0^{+50.0}_{-11.0}$ \\
              
% %         & $r_{out}$ ($r_g$) & 100000 (fixed) \\
% %         & $H_{tmax}$ ($r_g$) & $R_{hot}$ \\

% % In Figure 13 of the \cite{Czerny2003corona_highacc} and Figure 4 of the \cite{MN_BCZ_skin2004} we are able to see an absorption. However, in the case of J1105, neither mentioned approach is enough to explain such deep absorption. For this reason, the QSOSED model seems a good approach to parametrize the corona and disk well; moreover, the AGNSED seems an even better approach due to the free parameters of either the corona or the disk. 
% %other three seem to be important. I have decreased the number of the Gaussian functions in various variations but it always got worse

% % For clarity of the results it might not be used/included.

% % However, the redshift of the \CIV\ cloud along the line of sight indicates the existence of intervening systems \citep{Stone_abs_2019}. The ion column density calculation (see Sec \ref{sec:NH}) adds another argument in favor of the \CIV\ absorption material.

% %Calculation of Sec. \ref{sec:calc_abs}



% % Mrk 359 of \cite{Czerny2003corona_highacc} study has model parameters for Mrk 359 with warm skin, \mdotm 0.3,
% %for 19 degrees of freedom.

% % I have collected data to expand the sample of unordinary SMBH quasars from the SDSS catalog.

% % The reddening curve is steeper than in the SMC correction \citep{Meusinger2016}. Moreover, it is even steeper than the IRAS 14026+4341 case which was investigated broadly by \cite{Jiang_2013}. 

% % (pech chcial ze Meusinger nie za bardzo skupia sie na J1105, tlumaczy inne podobne kwazary jako sekcja 4.2.1, ale wprost o J1105 nic nie znalazlem.

% %\textbf{Meusinger mentioned J160827.08+075811.5 ( nr 6) resembles a weak-line quasar, but with an unusual broad emission structure shortwards of Mg II.}

% % \cite{Meusinger2016} indicated that J1105 has reddening steeper than in the Small Magellanic Cloud (SMC), perhaps even steeper than for IRAS 14026+4341. They could not either find a good reddening/extinction solution for the case of J1105. They classify it as strongly reddened narrow-line quasar.

% % BOSS spectrum displays strong narrow emission lines from Si IV, \CIV\, Al III, C III, and \MgII\ and an associated \MgII\ absorption line. 

% % Meusinger parameters: zem 1.929, zabs 1.925, $E^{smc}_{B-V}$ = 0.22, $E^{gask}_{B-V}$ = 0.13, log L, IR = 13.26 Lsun, L, 3000 Lsun = 13.19, R = <0.3.

% % \cite{Meusinger2016} the J1105 is in the sample of objects with reddening steeper than SMC extinction curve (or flatter). 

% % section 4.2.1. (Reddening with a steeper than SMC extinction curve) - as a hypothetical explanation of Meusinger 16, represents
% % Czy ten fit jest ok, czy lepiej nie pokazywac?

% % \begin{figure}[ht]
% %   \centering
% %     \includegraphics[width=1.0\textwidth]{figures/corona/J110511_meusinger_2019.png}
% %  \caption{Example from Meusinger 2016 - the J1105 fit.}
% % \end{figure}

% % Comptonization of a fraction of disk photons is clearly needed in order to reproduce the soft Xray part of the spectrum. In the high luminosity objects the disk extends down to the marginally stable orbit and some warm skin covers the inner region. Similar interpretation holds both for galactic black holes in their High State or Very High State and for luminous AGN (ref. [5,6]). Here we propose a natural constraint for the properties of this warm skin based on stability analysis
% % in the radiation pressure dominated region of the disk. We assume that the accretion disk is azimuthaly divided into two layers: inner cold part and a warm Comptonizing skin (Fig. 3). We futher assume that fraction of the energy is transported from the disk interior towards the skin as a magnetic flux. In this way proceed the heating

% % The skin cools predominantly by Comptonization. The cooling efficiency is fixed by the parameter w, i.e. the Compton amplification factor, A, is given by The role of the irradiation and the Comptonization by the warm absorber and disk skin is illustrated in Fig. 4. The model does not fit exactly the observed data points (Fig. 5) since our aim of our model is to reproduce in a possibly natural


% % AGNSED:MBHsolar 3.52232E+09 +/- 1.06453E+07
% % logmdot -0.561929 +/- 1.61374E-03
% % astar0.358481  +/- 2.13062E-02
% % cosi0.841001  +/- 2.80388E-03

% % QSOSED:

% % mass  solar 3.52246E+09 +/- 1.05220E+0
% % logmdot Ledd  -0.561976 +/- 1.59212E-03
% % asar 0.359667  +/- 2.00565E-02
% % cosi  0.840913  +/- 2.80587E-03



% % I have ruled out the three possibilities. I have used two different programs of the prof. BCz. Last but not least were the third possible extinction. It is based on the diamond explanation \citep{Wickramasinghe1998}. 

% %In this work the curve has a hyperbole shape.
% % It was applied for the my extinction procedure using 

% %for the \MgII\ $V$ (velocity) = - 139045 \kms\ and for the \CIV\ $V$ = - 9115 \kms. 
% % \begin{equation}
% %     \nu_{obs} = \nu_{em} \frac{c}{c+V},
% % \end{equation}
% % then after rearrangement:
% % \begin{equation}
% %     V = \frac{\nu_{em}c - \nu_{obs}c}{\nu_{obs}},
% % \end{equation}
% % the final equation for the velocity looks like:
% % \begin{equation}
% %     V = \frac{\frac{c}{\lambda_{em}}c - \frac{c}{\lambda_{obs}}c }{\frac{c}{\lambda_{obs}}}
% % \end{equation}
% % for the \MgII\ $V$ (velocity) = - 139045 \kms\ and for the \CIV\ $V$ = - 9115 \kms. 
% % \subsection{Determining the intrinsic speed in the absorber}
% % Assuming that the $\sigma$ from the Gaussian fit response for tis turbulent speed in the wind we are able to use the \FWHM\ relation where $\mFWHM = \sqrt{2ln2}\sigma \sim 2.35 \times \sigma$, then we can calculate the \FWHM:
% % \begin{equation}
% %     \frac{\mFWHM [\angstrom]}{\lambda_{em}[\angstrom]} = \frac{\mFWHM [\mkms]}{c [\mkms]}
% % \end{equation}
% % \noindent so the \FWHM\ for the J1105 is equal to 221.25 \kms.
% % As interpretation of the absorption the \MgII\ is inadequate. Whereas, the \CIV\ position indicates a plausible explanation and a good candidate for the absorber. The closer position of the \CIV\ line indicate more accurate explanation than the \MgII. The velocities can have either the positive or negative values. It depends on the fact if the medium is moving into observer or out of the observer and line of sight. 
% % \CIV\ is discussed in the \cite{Stone_abs_2019} work The Figure 3 of their paper represents the velocity distribution of \CIV\ absorption. Regarding the redshift which is calculated, I have ruled out the low-velocity intrinsic absorber which reached $\beta = V/c = 0.02$. The more plausible explanation either the high-velocity absorber or intervening system reach the maximum of $\beta = 0.10$.
% %Their classification indicate that ...
% % The delta z = 0.03 is rather intervening absorbers. If it is the case, the turbulent velocity indicated rather the other galaxy between us and the QSO than cold intergalactic cloud/s. The dispersion of velocity is around 20 \kms, not 200 \kms.

% %The optical depth at line center is par3/par2/$\sqrt{2\pi}$.
% % \begin{itemize}
% %     \item Line E(keV) = $2.239\times 10^{-3}  \pm 4.991\times 10^{-4}$
% %     \item $\sigma (keV) = 3.852\times 10^{-4} \pm 2.149 \times 10^{-4}$
% %     \item strength = $1.376\times 10^{-3}  \pm 5.565\times 10^{-3}$
% % \end{itemize}

% % The second Gaussian position:
% % \begin{itemize}
% %     \item Line E(keV) = $ 2.931\times 10^{-3}  \pm 9.247\times 10^{-4}$
% %     \item $\sigma (keV) = 4.931\times 10^{-4} \pm 6.119 \times 10^{-4}$
% %     \item strength = $ 2.561\times 10^{-3}  \pm 5.405\times 10^{-3}$
% % \end{itemize}

% %QSOS
%     % \hline
%     % \multirow{3}{*}{Third Gaussian} & Line E(keV) & $(1.823 \pm 0.008) \times 10^{-3}$\\
%     % \cline{2-3}
%     % & $\sigma$ (keV) & $(1.191 \pm 0.602)\times 10^{-5}$\\
%     % \cline{2-3}
%     % & strength & $(2.269 \pm 0.348) \times 10^{-6}$ \\
%     % \hline
%     % \multirow{3}{*}{Forth Gaussian} & Line E(keV) & $(2.125 \pm 0.029) \times 10^{-3}$\\
%     % \cline{2-3}
%     % &$\sigma$ (keV) & $(8.042\pm 2.666) \times 10^{-5}$\\
%     % \cline{2-3}
%     % &strength & $ (5.385 \pm 1.606) \times 10^{-5}$\\
%     % \hline
% %AGN
%     % \multirow{3}{*}{Third Gaussian} & Line E(keV) & $(1.823 \pm 0.008) \times 10^{-3}$\\
%     % \cline{2-3}
%     % & $\sigma$ (keV) & $(1.191 \pm 0.602)\times 10^{-5}$\\
%     % \cline{2-3}
%     % & strength & $(2.269 \pm 0.348) \times 10^{-6}$ \\
%     % \hline
%     % \multirow{3}{*}{Forth Gaussian} & Line E(keV) & $(2.125 \pm 0.029) \times 10^{-3}$\\
%     % \cline{2-3}
%     % &$\sigma$ (keV) & $(8.042\pm 2.666) \times 10^{-5}$\\
%     % \cline{2-3}
%     % &strength & $ (5.385 \pm 1.606) \times 10^{-5}$\\
    
    
% % \begin{table}[ht]
% %     \centering
% %     \caption{\textbf{redden*AGNSED*gabs*gabs} model parameters.}
% %     \begin{tabular}{|c|c|c|c|c|c|c|c|}
% %     \hline
% %     Parameter & Value & & Parameter & Value & & Parameter & Value \\
% %     \hline
% %     \hline
% %     {\mbh}(\Msun) & free & & cos {\incl}  & free & & $R_{hot}$ ($r_g$) &  $58.54 \pm  3.36$ \\
% %     \hline
% %     D (Mpc) & 5075 & & $kT_{e, hot}$ ( keV) & 100 (fixed)* & & $R_{warm}$ ($r_g$) & $430.0^{+50.0}_{-11.0}$  \\
% %     \hline
% %     {\dotm} & free & &  $kT_{e, warm}$ ( keV) & $0.356^{+4.876}_{-0.350}$ & & $r_{out}$ ($r_g$) & 100000 \\
% %     \hline
% %     {\as} & free & & $\Gamma_{hot}$ & $1.300^{+1.545}_{-1.300}$ & & $H_{tmax}$ ($r_g$) & $R_{hot}$ \\
% %     \hline
% %     E(B-V) & 0.08   & & $\Gamma_{warm}$ & $2.722 \pm 0.153$ & & z & free \\
% %     \hline
% %     \end{tabular}
% %     \label{tab:agnsed_parameters}
% %     \begin{quote}
% %     * - fixed according to \cite{KubotaDone_2018} assumptions
% %     \newline  NOTE: reprocess - ON
% %     \end{quote}
% % \end{table}


==> old_bayes.tex <==
Bayesian inference is the process of fitting a probability model to a set of data and summarizing
the result by a probability distribution on the parameters of the model and on
unobserved quantities such as predictions for new observations \citep{gelmanbda04_bayes}.

%https://www.mathsisfun.com/data/bayes-theorem.html
%https://www.investopedia.com/terms/b/bayes-theorem.asp
Bayes' Theorem describes the method of finding the probability which a certain knowledge of other probabilities.

The main formula is written as:
\begin{equation}
    P(A|B) = \frac{P(A) P(B|A)}{P(B)} ,
\end{equation}
where P(A|B) says how often A happens given that B happens; P(B|A) - our knowledge of how often B happens given that A happens, P(A) - how likely A is on its own, and P(B) - how likely B is on its own. In other word: P(A) is the probability of A occurring, P(B) is the he probability of B occurring. Whereas  P(A|B) is the probability of A given B and P(B|A) is the probability of B given A. 
Prior probability, in Bayesian statistical inference, is the probability of an event before new data is collected. (the best assessment of the probability of an outcome based on the current knowledge before an experiment is performed)

Posterior probability is the revised probability of an event occurring after taking into consideration new information. Posterior probability is calculated by updating the prior probability by using Bayes' theorem. In statistical terms, the posterior probability is the probability of event A occurring given that event B has occurred.


%P(A⋂B))= The probability of both A and B occurring

%--------------------------------------------------------------------
\textbf{Depend on the approach 1 or 2, signs of the A/B or I/H will change respectively.}

\textbf{Following is the description for the WLQs approach}
The Bayesian inference method requires the knowledge of the prior
probability distribution $P(H|I)$, which represents our beliefs about
a hypothesis $H$ before some evidence, $I$, is taken into account. In
this calculation $H$ is $j$th model, e.g $mod_j = mod(M_{\mathrm{BH} j},
\mdotm_j, a_{\ast j}, i_j)$, from among N models I put in.  Any prior information about this $j$th model is $I$. For instance prior observations of luminosity, \FWHM.

For each $j$th model, I have also derived its likelihood function $\mathcal{L}(mod_j) \propto \exp{(-\chi^2/2)} = P(D|mod_j,I)$, where $D$ is the set of photometric points measured for each WLQ
quasar. Note, that there is no free parameters.

The Bayesian analysis identifies a model which has the highest probability
of explaining the observed SED assuming knowledge of BH mass and
accretion rate.

Additionally, the black hole masses determined from the Bayesian analysis are presented in
Tab. \ref{tab:Bayes}. No significant differences in black hole masses calculated from both the $\chi^2$ and the Bayesian analysis
are indicated. It suggests that the determined global parameters are correct and describe
the overall SED shape of these objects. We take the values from Tab.~\ref{tab:bestfit} for further analysis.
\newpage
\textbf{The second approach}
In order to use information on yet determined data (e.g. black hole masses, accretion rates, and their errors in quasar sample) one can carry out a more sophisticated statistical analysis using the Bayesian method. It is the conditional distribution of the uncertain quantity given
the data. 
%_-------------------------------------------------------------
According to Bayes' theorem the posterior probability can be assign as:
\begin{equation}
   P(H|I) \frac{P(I|H) \cdot  P(H)}{P(I)}
\end{equation}
where $H$ is a hypothesis, which could be affected by data, $P(H)$ - a prior probability of an uncertain quantity that express one's beliefs before calculation. It defines(constrains) the information about a variable. $I$ is the evidence, connect with new data that were not included in calculation of $P(H)$. The posterior probability is define as $P(H|I)$, it is a probability of hypothesis given by evidence. The likelihood, the $P(I|H)$ is the probability of observing evidence given hypothesis. It measures the goodness of fit of a model to a data. It is assumed that likelihood function is a evidence function, whereas the posterior probability is a hypothesis function. $P(I)$ stand for "model evidence". It is the same for all possible hypothesis taking into account. This value is not consider into account for different hypotheses. 

==> old_ch1.tex <==
\chapter{Introduction}

\section*{Abstract \label{abstract_chapter1}}

Active galactic nuclei (AGN) provide unique tests of fundamental physics in regimes inaccessible on Earth and play an important role in our understanding of the evolution of galaxies. We describe these systems through the "Unified Model" in which AGN contains a central black hole (BH), an accretion disk (AD), jets, strong magnetic fields, and exhibit chaotic inflow processes. Modeling these components therefore requires understanding physical processes across a wide range of scales. While the Unified Model explains many of the peculiar behaviors of different types of AGN, they still fail to explain some classes such as \textbf{weak emission-line quasars (WLQs)}. 

% \section{History of the active galactic nuclei}

% The discovery of quasars (Schmidt 1963), Seyfert 1943 had reported the presence of broad and strong emission lines in the nuclei of six spiral nebula. 

\section{AGNs}
From hundreds of years we are looking at sky and observing the astonish nature of the cosmos. Recent decades shows many new discoveries about nature of AGNs. They are powered by accretion onto supermassive black holes, and we are able to observe their features across the full electromagnetic spectrum. From the zoo collection of all of the types of AGNs, thanks to recent study we are able to constrain them well. One of the main discrepancy/difference is the angle at which the observer sees the object. Currently, we are certain that the line of sight is crucial. The AGNs type are determine by the inclination angle \ref{fig:type_agn}. 

In the late 1970s studies of AGNs started. Long after the first discovery of quasi-stellar objects (QSOs) in the 1960s. Nowadays, all objects containing active SMBHs are refereed as AGNs. Two decades before that Carl Seyfert observed one of the first galaxies. In honor to him there are two types of Syfert galaxies, type 1, and typ 2. The main discrepency between theses two is in the optical-ultraviolet spectra. Seyfert 1 galaxies have strong and broad emission lines (2000 - 10 000 $\mkms$), whereas Seyfert 2 galaxies do not exceed width 1200 $\mkms$. Differences in the broadness is assigned as discrepency in the viewing angle to the central source. 

Due to the very energetic event -- accretion -- onto a central supermassive black hole (SMBH), AGN are stronger emitter than the nuclei of normal galaxies.
They have very high luminosities (up to $L_{bol} \approx 10^{45} - 10^{48}\mergs$) and emission across the whole electromagnetic spectrum. These features provide an excellent field for the astrophysical research of their nature.
% The main features of AGNs are:
% \begin{itemize}
%     \item very high luminosities (up to $L_{bol} \approx 10^{48} \mergs$)
%     \item
%     \item emission across the whole electromagnetic spectrum 
%     \item
% \end{itemize}

The multi-wavelength study of AGN provide many windows to observe their properties. The infrared (IR) band is sensitive to obscuring matter and dust. The optical and ultraviolet (UV) bands are related to the emission from the AD. The X-ray emission is assign mostly/putative to the corona.
According to \cite{Padovani17} review. The non-thermal emission is attribute to radio and $\gamma$ emission.

The Table 1 \cite{Padovani17} presents list of the AGN classes. In my thesis I have focused on the Quasars (quasi-stellar objects).

Even if the AGNs are one of the biggest objects in the whole Universe, in the description of their physics they are much simpler. Previously mentioned -- orientation; accretion rate' absence of presence of the jets, the environment within host galaxy. 

\begin{figure}[ht]
  \begin{center}
    \plotone{figures/ch1/type_agns.jpg}
  \end{center}
    \caption {Types of AGNs \citep{Antonucci2002}}
    \label{fig:type_agn}
\end{figure}

\begin{figure}[ht]
  \begin{center}
    \plotone{figures/ch1/padovani2017_SED.jpg}
  \end{center}
    \caption {AGN spectral energy distribution (SED). \citep{Padovani17}}
    \label{fig:padovani_sed}
\end{figure}

\ref{fig:padovani_sed} represent the schematic spectral energy distribution of AGN. Total emission is represents by the black solid curve, each of the components is represent by different color curves (for better clarity authors shifted it down).

The intrinsic shape of the SED in the mm-far infrared (FIR) regime is uncertain; however, it is widely believed to have a minimal contribution (to an overall galaxy SED) compared to star formation (SF), except in the most intrinsically luminous quasars and powerful jetted AGN. The primary emission from the AGN accretion disk peaks in the UV region. The jet SED is also shown for a high synchrotron peaked blazar (HSP, based on the SED of Mrk 421) and a low synchrotron peaked blazar (LSP, based on the SED of 3C 454.3; see Sect. 6.1). Adapted from Harrison (2014). 


\citet{Peterson97_book} Table 7.1 presents simplification of the Unification of AGN. Abbreviations: FIR galaxy -- far infrared; BL Lac -- BL Lacertae (rapid and large-amplitude flux variability and significant optical polarization) ;BLRG -- broad-line radio galaxies; NLRG -- narrow-line radio galaxies; OVV -- optically violently variable QSOs; FR (Fanaroff–Riley) class I and II. 

\begin{table}[ht]
  \centering
\begin{tabular}{lll}

\hline
\multicolumn{2}{c}{Orientation} \\
Face-On & Edge-On & Radio properties\\
\hline
Seyfert 1 & Seyfert 2 & Radio Quiet\\
QSO  & FIR galaxy & \\
\hline
 BL Lac & FR I & Radio Loud\\
 BLRG & NLRG & \\
 Quasar/OVV & FR II & \\
 \hline


\label{tab:AGN_unification_Peterson}
\end{tabular}
\caption{AGN Unification}
\end{table}

\subsection{My interest on the AGN emission}
The AGN emission is driven by accretion onto a SMBH. 

\subsection{The continuum of the accretion disk}
\textbf{before that should I write 1/2 pages about accretion overall? Like bondi accretion ,Eddington limit, Eddington luminosity?}

Peterson97: 
at least to a low-order approximation the SED of AGNs can be described as a power law of the form Fv propt niu to - lambda , where a is generally between zero and unity. This led to the initial suspicions that this continuum is non-thermal in origin. It is certainly tempting to attribute the bulk of an AGN spectrum to synchrotron emission, primarily because of the broad- band energy characteristics of the emission and because of the similarity of the spectra to known synchrotron sources such as supernova remnants and extended radio sources.

The SED of a quasar continuum approximately take the form of: $F_{\nu} = \nu^{-\alpha}$, with $0 \leq \alpha \leq 1$.

or \cite{Netzer13} $L_{\lambda} = \lambda^{-\beta}$, where $\alpha$ is the frequency spectral index $\beta$ is wavelength spectral index $\beta = 2 -\alpha$.
For example, the observed 1200-6000 Angs continuum of many luminous AGNs is described by 
$F_{\nu} \approx \nu^{-0.5}$, $L_{\lambda} = \lambda^{-1.5}$. This single powerlaw approximation clearly fails for wavelenght below 1200 or above 6000.

\cite{Peterson97_book} The big blue bump is generally agreed to be thermal in origin, although it is not clear whether it is optically thick (blackbody) or optically thin (free-free) emission. Many proponents of the optically thick interpretation ascribe the big blue bump to the purported accretion disk.

\textbf{worth noting: }There is a weaker feature superposed on the big blue bump between ~ 2000-4000 A, known as the 'small blue bump'. This feature is attributable to a combination of Balmer continuum emission and blends of Fe II emission lines arising in the broad-line region \citep{Peterson97_book}.

AGN spectrum contains the thermal and non-thermal emission. Thermal emission came from radiation due to particles (which have attained a Maxwellian velocity distribution) by collisions. Non-thermal emission comes form particle whose velocities are not described by a Maxwell-Boltzmann distribution (e.g. particles which give rise to synchrotron power-law spectra (since the kinetic energy distribution of these particles must also be a power-law)).
Emission is observe due to particles powered directly by central engine (e.g. synchrotron-emitting relativistic particles) or thermal emission from an AD (they are primary processes). Secondary instance is the emission by gas which receives its energy from the previous processes and re-radiates the emission (e.g. free-free emission from a photoionized or collisionally ionized gas)
\textbf{I could mention that} isotropy plays important role with determining of thermal vs non-thermal radiation. Synchrotron radiation; relativistic, non-thermal emission jets) if line of sight is close to axies of a jet, spectrum might be dominated by it since the emission is highly beamed in the direction of the electron motion, but the total amount of energy in the beam may be far less than that emitted by thermal processes, which is radiated isotropically. It distinguishes blazars from other AGNs.

The important observed features of a SED of the most AGNs are two bumps. One is the big blue bump which appears at around 4000 Angs.



\begin{figure}[ht]
  \begin{center}
    \plotone{figures/ch1/mean_qso_spec.png}
  \end{center}
    \caption {The mean QSO spectrum of 700 objects from the Large Bright Quasar Survey. Fig 2.\cite{Francis1991}, Fig 2.2 \cite{Peterson97_book}}
    \label{fig:mean_spec_qso}
\end{figure}

\textbf{should I compare Seyfert 1 and Seyfert 2 galaxies? Should I explude that WLQ cannot be Sy 2? e.g lines in Sy 2 are more prominent than in WLQ?, the ratio of OIII/Hbeta flux in much larger, in WLQs sometimes in not seen at all?, giant stars in the host galaxy in both Sy types, WLQs not really.}

For example: Seyfert 1.8 galaxies, the broad components are very weak, but detectable at H beta as well as H alpha.

Indeed, the AGN continuum is usually so weak in Seyfert 2 galaxies that it is very difficult to isolate it from the stellar continuum unambiguously.

The most luminous subclasses of AGNs family are the Quasars (with nuclear magnitudes Mb < -21.5+5 log h0. Around 10 \% of them are very strong radio sources (which the name Quasar orignially occured). The main difference between QSO and Seyfert galaxies is the spatiall resolution. According to the Palomor Sky Survey photographs it has angular size smaller than 7''. QSO spectra are very similar to Seyfert galaxies except that: stellar abosrption is weak or undetactable and the narrow lines are weaker relative to the broad lines than in the case in Seyfert galaxies \citep{Peterson97_book}.

\cite{Netzer13} main observational difference between Seyfert 1 and 2 galaxies is their different optical-ultraviolet spectra. Sy 1 show strong, very broad (2000 - 10000 \kms) permitted and semiforbidden emission lines. whereas the broadest lines in Sy2 have widths that do not exceed 1200 \kms. Such differences are now interpreted as arising from different viewing angles to the centers of such sources and from a large amoung of obsucration along the line of sight. . Typ 2, heavy obscuaration along the line of sight that extincts basically all the optical-IV radiation form the inner parsec. Type 1 for those sources with unobscured lines of sight to ther centers. 

\textbf{netzer 140, 220, + update of table with radio loud/quiter + update LBQS mean spectra?}

\subsection{Optical - UV continuum}
The big blue bump which is a crucial feature in the optical/UV AGNs spectra is attributed as thermal emission in the range of $10^5-10^6$ Kelvins. The temperature depends of the emission area either an optically thin or thick region.
\cite{Peterson97_book} pointed out that if we assume the black hole mass as $10^8 \mMsun$ which accreating at the Eddington rate, the emission form the inner part of the disk is maximed at a frequency $3.6\times10^16$ Hz which corresponds to 100 \angstrom or 100 eV. It indicates the maximum of the optical/UV emission from AD (i.e big blue bump).

One can assume that the AD radiates like a blackbody:
\begin{equation}
    B_{\nu} = \frac{2h\nu^3}{c^2}\frac{1}{e^\frac{h\nu}{kT(r)}-1}
    \label{Planck_eq}
\end{equation}
where T(r) is a disk temperature at radius from the center.

\textbf{I am wondering about putting the Eddington rate, Luminosity of a disk as $L_{\nu}$, what do you think?}

\textbf{Peterson book, should I include it?}We consider as an example a $10^8 \mMsun$ black hole that is accreting at the Eddington rate (i.e., a luminosity L « 1046 ergs s 1 QSO). Equations (3.21) and (3.18) show that the peak contribution to the 1500 A continuum arises at r « 50Rs, i-e., around 1.4 x 1015cm or 0.6 light days from the black hole. The peak contribution to the 5000A continuum, however, arises at r « 240 R, i-e> around 7.1 x 1015cm or 2.8 light days.

\begin{figure}[ht]
  \begin{center}
    \plotone{figures/ch1/plot_AD.jpg}
  \end{center}
    \caption {}
    \label{}
\end{figure}


% AGN accretion has historically been modeled as occurring through geometrically thin, optically thick accretion disks (Novikov & Thorne 1973; Shakura & Sunyaev1973). 
% Such disk models are thermally unstable at small
% radii where radiation pressure dominates (Shakura &
% Sunyaev 1976; Shapiro et al. 1976), although radiationmagnetohydrodynamics simulations indicate that they
% may be stabilized by magnetic pressure or convectiondriven turbulence (Jiang & Blaes 2020; Jiang et al.
% 2019a,b). Additionally, standard thin accretion disk
% models (Shakura & Sunyaev 1973) become gravitationally unstable at large radii, and multiple methods of
% taking this into account have been suggested (Sirko &
% Goodman 2003; Thompson et al. 2005).
\section{WLQ}

Quasars were originally discovered as a result of the first radio surveys of the sky in the late 1950s.

WLQs, \textbf{an unsolved puzzle} has equivalent width (EW) of CIV below 10\AA\ and weak or lack of the Lyman $\alpha$ emission \citep{DS09}. WLQ theories provide a few hypotheses of their nature: radiatively inefficient accretion flow \citep{Yuan04}, a cold accretion disk with a small accretion rate \citep{Laor11}, an extremely high accretion rate \citep{Leighly07a} \citep{Leighly07b}, the presence of shielding gas between the AD and a broad line region (BLR) \citep{Wu11} or an unusual BLR \citep{Shemmer10} \citep{Nikolajuk12}. Several works about X-ray properties of WLQs have recently appeared\citep{Ni18} \citep{Tim20}, \citep{Pu20}. The conclusion arising is that WLQs are more likely to be X-ray weaker (about half of them) than normal quasars. Luo et al.\citep{Luo15} suggest that it may be caused by the shielding gas, which prevents the observer from seeing the central X-ray emitting region. 

Weak emission-line quasars (WLQs) are an unsolved puzzle in the model of active galactic nuclei (AGN).  The typical equivalent width (\EW) of the \CIV\ emission line is extremely weak ($\la 10{\angstrom}$) compared to normal quasars and very weak or absent in Ly$\alpha$ emission \citep{Fan99,DS09}. \citet{DS09} concluded that WLQs have optical continuum properties similar to normal quasars, although Ly$\alpha$+\NV\ line luminosities are significantly weaker, by a factor of 4. An explanation for the weak or absent emission lines has not be found so far. Probable explanations include a radiatively inefficient accretion flow \citep{Yuan04} and a cold accretion disk \citep{Laor11} with a small accretion rate.  An extremely high accretion rate where we have inefficient photoionized flux is proposed by \citet{Leighly07a,Leighly07b}. Parallel to that \citet{Wu11} postulate presence of shielding gas between the accretion disk and a broad line region (BLR), which could absorb the high-energy ionizing photons from the accretion disk.  The last (the latter?) model suggests an unusual BLR i.e., anemic in construction and gas abundance \citep{Shemmer10, Nikolajuk12}. This explanation supports the idea that WLQs can also be in the early stage of AGN evolution \citep{Hryniewicz10, Liu11, Banados14, Meusinger14}.  Several works about X-ray properties of WLQs have recently appeared \citep[e.g.][]{Wu11,Wu12,Ni18, Marlar18}.  
The conclusion arising from these works is that WLQs are more likely to be X-ray weaker (about half of them) than normal quasars. For example, \citet{Ni18} mentioned that 7 of the 16 WLQs in their sample are X-ray weak. \citet{Luo15} suggested that it may be caused from the shielding gas which prevents the observer from seeing the central X-ray emitting region.

Knowledge about the values of black hole (BH) masses and the accretion rates is crucial in understanding an accretion flows phenomena. The most robust technique is the reverberation mapping method \citep[RM,][]{Blandford82, Peterson93, Peterson14, Fausnaugh17, Bentz18, Shen19}. This method is based on the study of the dynamics surrounding the black hole gas. In this way, we are able to determine
the supermassive black hole (SMBH) mass:
\begin{equation}
    \mmbh = 
    \frac{v^2_{\mathrm{BLR}} R_{\mathrm{BLR}}}{G} =
    f \frac{\mathrm{\FWHM}^2 R_{\mathrm{BLR}}}{G}
\label{eq:blr}    
\end{equation}
where \mbh\ is the black hole mass, G is the gravitational constant, $R_{\mathrm{BLR}}$ is the distance between the SMBH and a cloud in the broad line region (BLR), and $v_{\mathrm{BLR}}$ is a velocity of the cloud inside the BLR.  This speed is unknown and we express our lack of knowledge in the form of the Full Width Half Maximum (\FWHM) of an emission-line and $f$ - the virial factor, which describes a distribution of the BLR clouds. In the RM the $\mRblr$\ is determined as the time delay between the continuum change and the BLR response. This technique requires a significant number of observations.  The modification of this method is the single-epoch virial BH mass estimator \citep[see][for review]{Shen13}.  The correlation between $\mRblr$ and continuum luminosity ($\nu L_\nu$) is observed \citep{Kaspi05, Bentz09} and incorporated in Eq.~(\ref{eq:blr}).  Thus, the method is powerful and eagerly used because of its simplicity \citep{Kaspi2000, Peterson04, Vestergaard06, Plotkin15}. The nondynamic method, which is the spectra disk-fitting method, is based on well grounded model of emission from an accretion disk (AD) surrounded black hole \citep[e.g.][]{SS73, NT73}. The most important parameter in such models is the mass of the black hole and the accretion rate. The spin of the black hole and the viewing angle are also taken into account.  In this technique, a spectral energy distribution (SED) of an AGN is fitted to the
model and one is able to constrain these four parameters.  More advanced disk spectra models, which take into account an irradiation
effect, limb-darkening/brightening effects, the departure from a blackbody due to radiative transfer in the disk atmosphere, the
ray-tracing method to incorporate general relativity effects in light propagation, can be fitted \citep[e.g.][]{Hubeny2000, Loska04, Sadowski09, Czerny11HNS, Laor11,Czerny19BLRscaling}. Generally, the RM and the single-epoch virial BH mass method are inadequate for BH mass estimation in WLQs, due to weakness of emission-lines  in these objects.

\begin{figure}[ht]
  \begin{center}
    \plotone{figures/ch1/blr2.jpg}
  \end{center}
    \caption {WLQs hypothesis}
    \label{}
\end{figure}

\begin{figure}[ht]
  \begin{center}
    \plotone{figures/ch1/agn.jpg}
  \end{center}
    \caption {}
    \label{I will change labels if I will use this plot}
\end{figure}
% ---------------------------------------------------------------

{\bibliographystyle{apj}}
% NOTE: you list the .bib files referenced here, in our case,
%       we reference bib_sample.bib
{\bibliography{apj}}


==> plots_SED_Old.tex <==
% \begin{figure}
% \centering
% \subfloat[first]{
%   \includegraphics[width=65mm]{figures/ch5/J0836_May_done.pdf}}
%   \caption{}\label{fig:J0836}

% \subfloat[second]{
%   \includegraphics[width=65mm]{figures/ch5/J0945_revison_mirror4.pdf}
% }
% \caption{J0945} \label{fig:J0945}
% \hspace{0mm}
% \subfloat[third]{
%   \includegraphics[width=65mm]{figures/ch5/J1141_revision_csv.pdf}
% }
% \caption{J1141} \label{fig:J1141}
% \subfloat[forth]{
%   \includegraphics[width=65mm]{figures/ch5/J1237_revision_csv_CUT.pdf}
% }
% \caption{J1237} \label{fig:J1237}
% \hspace{0mm}
% \subfloat[]{   % ???
%   \includegraphics[width=65mm]{empty.pdf}
% }
% \subfloat[fifth]{
%   \includegraphics[width=65mm]{test.pdf}
% }
% \caption{caption}
% \end{figure}



% \begin{figure}[t]
% \centering
    
%     \plotone{figures/ch5/J0836_May_done.pdf}

% \caption{J0836 \textbf{labels x, y will be update, I will make all plots the same, with labels and legend. I will make 2 plots per page}}
% \label{fig:J0836}

% \centering
    
%     \plotone{figures/ch5/J0945_revison_mirror4.pdf}

% \caption{J0945}
% \label{fig:J0945}

% \centering
    
%     \plotone{figures/ch5/J1141_revision_csv.pdf}

% \caption{J1141}
% \label{fig:J1141}

% \centering
    
%     \plotone{figures/ch5/J1237_revision_csv_CUT.pdf}

% \caption{J1237}
% \label{fig:J1237}

% \end{figure}
% \clearpage

% \begin{figure}[t]
%   \begin{center}
    
%     \plotone{figures/ch5/J0945_revison_mirror4.pdf}
%   \end{center}
% \caption{J0945}
% \label{fig:J0945}
% \end{figure}



% \begin{figure}[t]


% \end{figure}
% \clearpage


% \begin{figure}[t]
%   \begin{center}
    
%     \plotone{figures/ch5/J1237_revision_csv_CUT.pdf}
%   \end{center}
% \caption{J1237}
% \label{fig:J1237}
% \end{figure}

\begin{figure}[t]
\centering
    
    \plotone{figures/ch5/J1411_revision_csv.pdf}

\caption{J1411}
\label{fig:J1411}
\centering
    
    \plotone{figures/ch5/J1417_revision_csv_2.pdf}

\caption{J1417}
\label{fig:J1417}

\end{figure}

% \begin{figure}[t]
%   \begin{center}
    
%     \plotone{figures/ch5/J1417_revision_csv_2.pdf}
%   \end{center}
% \caption{J1417}
% \label{fig:J1417}
% \end{figure}

\clearpage

\begin{figure}[t]
  \centering
    \plotone{figures/ch5/J1447_revision_csv.pdf}
\caption{J1447}
\label{fig:J1447}

  \centering
    
    \plotone{figures/ch5/J1521_revision_csv.pdf}
\caption{J1521}
\label{fig:J1521}

\end{figure}

% \begin{figure}[t]
%   \begin{center}
    
%     \plotone{figures/ch5/J1521_revision_csv.pdf}
%   \end{center}
% \caption{J1521}
% \label{fig:J1521}
% \end{figure}

\clearpage

\begin{figure}[t]
\centering
    
    \plotone{figures/ch5/PHL1811_revision_csv.pdf}

\caption{PHL1811}
\label{fig:PHL1811}

\centering
  
    \plotone{figures/ch5/PG1407_revision_csv.pdf}

\caption{PG1407}
\label{fig:PG1407}

\end{figure}

% \begin{figure}[t]
%   \begin{center}
  
%     \plotone{figures/ch5/PG1407_revision_csv.pdf}
%   \end{center}
% \caption{PG1407}
% \label{fig:PG1407}
% \end{figure}



\begin{figure}[htp]
  \centering
  \label{figur}\caption{equation...}

  \subfloat[Subcaption 1]{\label{figur:1}\includegraphics[width=60mm]{figures/ch5/J0836_May_done.pdf}}
  \subfloat[Subcaption 2]{\label{figur:2}\includegraphics[width=60mm]{figures/ch5/J0945_revison_mirror4.pdf}}
  \\
  \subfloat[Subcaption 3]{\label{figur:3}\includegraphics[width=60mm]{figures/ch5/J1141_revision_csv.pdf}}
  \subfloat[Subcaption 4]{\label{figur:4}\includegraphics[width=60mm]{J1237_revision_csv_CUT.pdf}}


\end{figure}


\includegraphics[width=0.45\textwidth]{figures/ch5/J0836_May_done.pdf}
%             \includegraphics[width=0.45\textwidth]{figures/ch5/J0945_revison_mirror4.pdf}
%             \includegraphics[width=0.45\textwidth]{figures/ch5/J1141_revision_csv.pdf}
%             \includegraphics[width=0.45\textwidth]{figures/ch5/J1237_revision_csv_CUT.pdf}

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.3\textwidth}
%         \includegraphics[width=\textwidth]{figures/ch5/J0836_May_done.pdf}
%         \caption{A gull}
%         \label{fig:gull}
%     \end{subfigure}\quad
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%       %(or a blank line to force the subfigure onto a new line)
%     \begin{subfigure}[b]{0.3\textwidth}
%         \includegraphics[width=\textwidth]{figures/ch5/J0945_revison_mirror4.pdf}
%         \caption{A tiger}
%         \label{fig:tiger}
%     \end{subfigure}\quad
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%     %(or a blank line to force the subfigure onto a new line)
%     \begin{subfigure}[b]{0.3\textwidth}
%         \includegraphics[width=\textwidth]{figures/ch5/J1141_revision_csv.pdf}
%         \caption{A mouse}
%         \label{fig:mouse}
%     \end{subfigure}\quad
%     \caption{Pictures of animals}\label{fig:animals}
%      \begin{subfigure}[b]{0.3\textwidth}
%         \includegraphics[width=\textwidth]{figures/ch5/J1237_revision_csv_CUT.pdf}
%         \caption{A mouse}
%         \label{fig:mouse}
%     \end{subfigure}\quad
%     \caption{Pictures of animals}\label{fig:animals}
% \end{figure}

==> tables/chapter5/bayesian_solutions_old.tex <==
  \begin{table}
  % \tablenum{6}
    \centering
    \caption {The BH masses from the Bayesian analysis (\as $\neq$0)}
    \begin{tabular}{cc}
    \hline   
    Name & \mbhbay\ [\Msun]\\
    \hline
    J0836 & $(2.00^{+4.30}_{-1.00})\times 10^9$ \\
    J0945 & $(3.20^{+3.10}_{-1.20})\times 10^9$ \\
    J1141 & $(7.90^{+4.10}_{-2.90})\times 10^9$ \\
    J1237 & $(6.30^{+3.70}_{-1.30})\times 10^9$ \\
    J1411 & $(1.30^{+1.90}_{-1.30})\times 10^9$ \\
    J1417 & $(2.50^{+2.50}_{-1.20})\times 10^9$ \\
    J1447 & $(1.00^{+1.50}_{-6.00})\times 10^9$ \\
    J1521 & $(1.30^{+1.20}_{-5.00}) \times 10^{10}$ \\
    PHL 1811 & $(7.90^{+3.10}_{-3.90}) \times 10^8$ \\
    PG 1407 & $(7.90^{+3.40}_{-2.90}) \times 10^9$ \\
    \hline
    \label{tab:Bayes}
    \end{tabular}
   \end{table}
   
   
    %   J0836 & $(2.00^{+4.30}_{-1.00})\times 10^9$ & $(0.32^{+0.31}_{-0.19})$ & $(0.3^{+0.6}_{-0.3})$ & $(0.91^{+0.39}_{-0.91})$ \\
    % J0945 & $(3.20^{+3.10}_{-1.20})\times 10^9$ & $(0.25^{+0.22}_{-0.18})$ & $(0.3^{+0.6}_{-0.3})$ & $(0.78^{+0.52}_{-0.78})$ \\
    % J1141 & $(7.90^{+4.10}_{-2.90})\times 10^9$ & $(0.39^{+0.45}_{-0.19})$ & $(0.4^{+0.4}_{-0.4})$ & $(0.78^{+0.52}_{-0.78})$\\
    % J1237 & $(6.30^{+3.70}_{-1.30})\times 10^9$ & $(0.27^{+0.33}_{-0.26})$ & $(0.4^{+0.5}_{-0.4})$ & $(0.78^{+0.52}_{-0.78})$\\
    % J1411 & $(1.30^{+1.90}_{-1.30})\times 10^9$ & $(0.48^{+0.51}_{-0.28})$ & $(0.4^{+0.5}_{-0.4})$ & $(0.78^{+0.52}_{-0.78})$\\
    % J1417 & $(2.50^{+2.50}_{-1.20})\times 10^9$ & $(0.32^{+0.41}_{-0.31})$ & $(0.3^{+0.6}_{-0.3})$ & $(0.78^{+0.52}_{-0.78})$\\
    % J1447 & $(1.00^{+1.50}_{-6.00})\times 10^9$ & $(0.37^{+0.50}_{-0.23})$ & $(0.6^{+0.3}_{-0.5})$ & $(0.78^{+0.52}_{-0.78})$\\
    % J1521 & $(1.30^{+1.20}_{-5.00}) \times 10^{10}$ & $(1.27^{+1.50}_{-0.82})$ & $(0.4^{+0.5}_{-0.4})$ & $(0.78^{+0.52}_{-0.78})$\\
    % PHL 1811 & $(7.90^{+3.10}_{-3.90}) \times 10^8$ & $(0.40^{+0.14}_{-0.05})$ & $(0.1^{+0.3}_{-0.1})$ & $(0.26^{+0.52}_{-0.26})$\\
    % PG 1407 & $(7.90^{+3.40}_{-2.90}) \times 10^9$ & $(0.29^{+0.25}_{-0.13})$ & $(0.8^{+0.1}_{-0.2})$ & $(0.78^{+0.52}_{-0.78})$\\

==> tables/ex_ch3/table_UKIRT_BS.tex <==
% $Id: table_UKIRT_BS.tex,v 1.1 2001/04/16 01:56:11 jim Exp $
%
% Table of UKIRT Faint Standards from March3  of 1992
%

\begin{sidewaystable}
\caption{UKIRT Bright Standards, March 3, 1992.
  Information is from the UKIRT Web site.
  \label{table_UKIRT_BS}}
\vspace{1ex}
\noindent
\begin{center}
\begin{tabular}{|r|l|c|r|r|r|r|r|r|r|r|r|r|}
\hline\extravspace
 & & &\multicolumn{3}{c|}{R.A. (J1950.0)} &\multicolumn{3}{c|}{Dec. (J1950.0)}&&&& \\
 No. & Name & Sp & h & m & s & \arcdeg & \arcmin & \arcsec & $J$ & $H$
 & $K$ & $K^{\prime}$ $^\dag$ \\
\hline\extravspace
   1   &
 $^\ddag$HD 225023 &A0        &00 &00 &11.8 & 35  &32 &14   &7.082  &6.993  &6.962   &6.970\\
   2   &
 $^\ddag$G158-27   &M5        &00 &04 &12.0 &-07  &47 &54   &8.378  &7.781  &7.447   &7.536\\
   3   &
 $^\ddag$BS 33     &F7V       &00 &08 &43.2 &-15  &44 &32   &3.964  &3.689  &3.636   &3.650\\
   4   &
 $^\ddag$HD 1160   &A0        &00 &13 &23.1 & 03  &58 &24   &7.060  &7.051  &7.040   &7.043\\
   5   & HD 2811    &A2        &00 &28 &53.0 &-43  &52 &58   &7.178  &7.093  &7.067   &7.074\\
   6   & HD 3029    &A3        &00 &31 &02.3 & 20  &09 &30   &7.263  &7.125  &7.093   &7.101\\
   7   & BS 337     &M0III     &01 &06 &55.5 & 35  &21 &22   &-0.908 &-1.70  &-1.85   &-1.813\\
   8   & BS 696     &B2Iae     &02 &21 &43.1 & 56  &23 &04   &5.587  &5.499  &5.443   &5.458\\
   9   &
 $^\ddag$BS 718    &B9III     &02 &25 &29.8 & 08  &14 &13   &4.374  &4.390  &4.390   &4.390\\
   10  & BS 739     &gG3       &02 &29 &36.6 &-01  &15 &17   &3.748  &3.218  &3.121   &3.147\\
   11  & BS 740     &F4IV      &02 &29 &43.0 &-15  &27 &48   &3.879  &3.623  &3.585   &3.595\\
   12  &
 $^\ddag$GL 105.5  &M0        &02 &38 &07.6 & 00  &58 &57   &7.305  &6.663  &6.539   &6.572\\
   13  & BS 816     &gF0       &02 &42 &43.4 & 04  &30 &08   &5.502  &5.384  &5.353   &5.361\\
   14  & HD 18881   &A0        &03 &00 &20.5 & 38  &12 &53   &7.130  &7.135  &7.140   &7.139\\
   15  & HD 19904   &A2        &03 &08 &49.1 &-39  &14 &24   &6.727  &6.662  &6.642   &6.647\\
   16  & G77-31     &M4?       &03 &10 &40.5 & 04  &35 &12   &8.816  &8.187  &7.857   &7.944\\
   17  &
 $^\ddag$HD 22686  &A0        &03 &36 &18.7 & 02  &36 &07   &7.196  &7.190  &7.185   &7.186\\
   18  & BS 1140    &B7IV      &03 &41 &49.5 & 24  &08 &01   &5.520  &5.500  &5.510   &5.507\\
   19  & BS 1457    &K5III     &04 &33 &02.9 & 16  &24 &37   &-1.848 &-2.61  &-2.78   &-2.738\\
   20  & BS 1543    &F6V       &04 &47 &07.4 & 06  &52 &32   &2.353  &2.117  &2.095   &2.101\\
   21  & BS 1552    &B2III     &04 &48 &32.4 & 05  &31 &16   &4.029  &4.087  &4.138   &4.124\\
   22  & BS 1641    &B7V       &05 &03 &00.2 & 41  &10 &08   &3.518  &3.646  &3.677   &3.669\\
   23  & BS 1637    &F0V       &05 &06 &40.6 & 51  &35 &52   &4.312  &4.204  &4.153   &4.167\\
   24  & BS 1713    &B8Iae     &05 &12 &08.0 &-08  &15 &29   &0.240  &0.241  &0.211   &0.219\\
\hline
\multicolumn{13}{|r|}{\extravspace\it continued on the next page}\\
\hline
\multicolumn{13}{l}{\extravspace
\llap{$^\dag$}{$K'=K+0.265*(H-K)$}
}\\
\multicolumn{13}{l}{
\llap{$^\ddag$}{multiple star system}
}
\end{tabular}
\end{center}
\end{sidewaystable}


\begin{sidewaystable}
\begin{center}
Table~\ref{table_UKIRT_BS}, continued.\hfill\\[2ex]
\begin{tabular}{|r|l|c|r|r|r|r|r|r|r|r|r|r|}
\hline\extravspace
 & & &\multicolumn{3}{c|}{R.A. (J1950.0)} &\multicolumn{3}{c|}{Dec. (J1950.0)}&&&& \\
 No. & Name & Sp & h & m & s & \arcdeg & \arcmin & \arcsec & $J$ & $H$
 & $K$ & $K^{\prime}$ $^\dag$ \\
\hline\extravspace
   25  & BS 1708    &G4III     &05 &12 &59.5 & 45  &56 &58   &-1.334 &-1.71  &-1.80   &-1.779\\
   26  & SAO112626  &F8        &05 &16 &41.4 & 01  &39 &15   &8.934  &8.670  &8.596   &8.616\\
   27  & BS 1869    &dF0       &05 &36 &15.9 & 47  &42 &56   &5.532  &5.454  &5.393   &5.409\\
   28  & HD 38921   &A0        &05 &45 &41.0 &-38  &14 &51   &7.572  &7.551  &7.536   &7.540\\
   29  &
 $^\ddag$HD 40335  &A0        &05 &55 &37.6 & 01  &51 &09   &6.555  &6.473  &6.452   &6.458\\
   30  & BS 2228    &F0V       &06 &17 &34.6 & 46  &25 &57   &6.012  &5.943  &5.892   &5.906\\
   31  &
 $^\ddag$HD 44612  &A0        &06 &21 &09.7 & 43  &34 &35   &7.075  &7.041  &7.041   &7.041\\
   32  & BS 2491    &A1V       &06 &42 &56.7 &-16  &38 &46   &-1.300 &-1.31  &-1.32   &-1.320\\
   33  &
 $^\ddag$BD+0 1694 &?         &06 &52 &07.3 & 00  &00 &52   &5.750  &4.857  &4.606   &4.673\\
   34  & BS 2721    &G0V       &07 &12 &07.6 & 47  &19 &51   &4.475  &4.180  &4.126   &4.140\\
   35  & BS 2943    &F5IV      &07 &36 &41.1 & 05  &21 &16   &-0.437 &-0.56  &-0.64   &-0.624\\
   36  & BS 2990    &K0IIIb    &07 &42 &15.6 & 28  &08 &55   &-0.523 &-0.97  &-1.05   &-1.030\\
   37  & BS 3314    &A0V       &08 &23 &09.7 &-03  &44 &31   &3.920  &3.919  &3.940   &3.934\\
   38  & HD 75223   &A0        &08 &45 &29.8 &-39  &36 &54   &7.329  &7.296  &7.281   &7.285\\
   39  &
 $^\ddag$HD 77281  &A2        &08 &59 &05.4 &-01  &16 &45   &7.111  &7.052  &7.031   &7.037\\
   40  &
 $^\ddag$GL 347A   &M3.5      &09 &26 &25.0 &-07  &08 &30   &8.483  &7.881  &7.658   &7.717\\
   41  &
 $^\ddag$HD 84800  &A2        &09 &45 &35.9 & 43  &53 &56   &7.592  &7.549  &7.538   &7.541\\
   42  & BS 3888    &F2IV      &09 &47 &27.1 & 59  &16 &30   &3.162  &3.005  &2.983   &2.989\\
   43  & BS 3903    &G7III     &09 &49 &04.3 &-14  &36 &40   &2.617  &2.136  &2.050   &2.073\\
   44  & V 569      &M3        &10 &09 &46.3 &-03  &29 &41   &5.992  &5.310  &5.106   &5.160\\
   45  & BS 4069    &M0III     &10 &19 &21.5 & 41  &45 &06   &0.132  &-0.65  &-0.80  -&0.764\\
   46  & GL 390     &M1.5      &10 &22 &44.0 &-09  &58 &36   &6.939  &6.275  &6.061   &6.118\\
   47  & GL 406     &M6        &10 &54 &06.0 & 07  &19 &12   &7.143  &6.469  &6.099   &6.197\\
   48  & BS 4358    &K3III     &11 &11 &25.9 & 08  &20 &05   &3.879  &3.299  &3.202   &3.228\\
\hline
\multicolumn{13}{|r|}{\extravspace\it continued on the next page}\\
\hline
\multicolumn{13}{l}{\extravspace
\llap{$^\dag$}{$K'=K+0.265*(H-K)$}
}\\
\multicolumn{13}{l}{
\llap{$^\ddag$}{multiple star system}
}
\end{tabular}
\end{center}
\end{sidewaystable}


\begin{sidewaystable}
\begin{center}
Table~\ref{table_UKIRT_BS}, continued.\hfill\\[2ex]
\begin{tabular}{|r|l|c|r|r|r|r|r|r|r|r|r|r|}
\hline\extravspace
 & & &\multicolumn{3}{c|}{R.A. (J1950.0)} &\multicolumn{3}{c|}{Dec. (J1950.0)}&&&& \\
 No. & Name & Sp & h & m & s & \arcdeg & \arcmin & \arcsec & $J$ & $H$
 & $K$ & $K^{\prime}$ $^\dag$ \\
\hline\extravspace
   49  & HD101452   &A2        &11 &37 &45.1 &-38  &52 &09   &7.018  &6.890  &6.848   &6.859\\
   50  & Y 2730     &dM4.5     &11 &45 &08.2 & 01  &05 &56   &6.532  &5.935  &5.646   &5.723\\
   51  & BS 4550    &G8V       &11 &50 &06.2 & 38  &04 &39   &4.957  &4.466  &4.400   &4.417\\
   52  & HD105601   &A2        &12 &06 &56.1 & 38  &54 &39   &6.821  &6.719  &6.687   &6.695\\
   53  &
 $^\ddag$HD106965  &A2        &12 &15 &24.0 & 01  &51 &10   &7.380  &7.337  &7.316   &7.322\\
   54  &
 $^\ddag$BS 4689   &A2IV      &12 &17 &20.8 & 00  &23 &21   &3.810  &3.781  &3.781   &3.781\\
   55  & BS 4935    &F7V       &13 &01 &05.1 &-20  &18 &55   &4.604  &4.290  &4.266   &4.272\\
   56  & BS 4983    &G0V       &13 &09 &32.5 & 28  &07 &52   &3.194  &2.929  &2.886   &2.897\\
   57  & BS 5340    &K1IIb     &14 &13 &22.8 & 19  &26 &31   &-2.200 &-2.87  &-2.97   &-2.950\\
   58  &
 $^\ddag$BS 5447   &F2V       &14 &32 &30.2 & 29  &57 &41   &3.723  &3.522  &3.489   &3.498\\
   59  & HD129653   &A2        &14 &40 &38.2 & 36  &58 &07   &6.985  &6.942  &6.921   &6.927\\
   60  &
 $^\ddag$HD129655  &A2        &14 &41 &11.0 &-02  &17 &38   &6.826  &6.724  &6.692   &6.700\\
   61  & HD130163   &A0        &14 &44 &36.2 &-39  &43 &04   &6.856  &6.846  &6.835   &6.838\\
   62  & BD+3 2954  &M0        &14 &52 &23.2 & 03  &11 &33   &5.926  &5.026  &4.825   &4.878\\
   63  & BS 5685    &B8V       &15 &14 &18.7 &-09  &11 &59   &2.759  &2.789  &2.799   &2.796\\
   64  &
 $^\ddag$HD136754  &A0        &15 &19 &24.3 & 24  &31 &19   &7.155  &7.146  &7.135   &7.138\\
   65  &
 $^\ddag$BD+2 2957 &K2        &15 &22 &29.0 & 01  &41 &06   &5.280  &4.454  &4.263   &4.314\\
   66  & BS 6084 B2 &II+O9V    &16 &18 &08.7 &-25  &28 &29   &2.491  &2.442  &2.421   &2.427\\
   67  &
 $^\ddag$BS 6092   &A9III     &16 &18 &14.1 & 46  &25 &54   &4.192  &4.257  &4.298   &4.287\\
   68  & S-R 3      &?         &16 &23 &07.7 &-24  &27 &26   &7.804  &7.001  &6.543   &6.664\\
   69  & OPH S1     &?         &16 &23 &32.8 &-24  &16 &44   &9.007  &7.344  &6.378   &6.634\\
   70  & BS 6136    &K4III     &16 &26 &00.9 & 00  &46 &32   &2.898  &2.184  &2.036   &2.075\\
   71  & BS 6147    &G8IIIa    &16 &28 &16.4 &-16  &30 &19   &2.767  &2.334  &2.269   &2.286\\
   72  & BS 6406    &M5Ib      &17 &12 &22.0 & 14  &26 &45   &-2.276 &-3.11  &-3.35   &-3.287\\
\hline
\multicolumn{13}{|r|}{\extravspace\it continued on the next page}\\
\hline
\multicolumn{13}{l}{\extravspace
\llap{$^\dag$}{$K'=K+0.265*(H-K)$}
}\\
\multicolumn{13}{l}{
\llap{$^\ddag$}{multiple star system}
}
\end{tabular}
\end{center}
\end{sidewaystable}

\begin{sidewaystable}
\begin{center}
Table~\ref{table_UKIRT_BS}, continued.\hfill\\[2ex]
\begin{tabular}{|r|l|c|r|r|r|r|r|r|r|r|r|r|}
\hline\extravspace
 & & &\multicolumn{3}{c|}{R.A. (J1950.0)} &\multicolumn{3}{c|}{Dec. (J1950.0)}&&&& \\
 No. & Name & Sp & h & m & s & \arcdeg & \arcmin & \arcsec & $J$ & $H$
 & $K$ & $K^{\prime}$ $^\dag$ \\
\hline\extravspace
   73  & HD161743   &A0        &17 &45 &31.8 &-38  &06 &11   &7.620  &7.620  &7.615   &7.616\\
   74  &
 $^\ddag$HD161903  &A2        &17 &45 &43.3 &-01  &47 &34   &7.172  &7.059  &7.023   &7.033\\
   75  &
 $^\ddag$HD162208  &A0        &17 &46 &20.7 & 39  &59 &40   &7.223  &7.141  &7.112   &7.120\\
   76  & BS 6707    &F2II      &17 &56 &35.3 & 30  &11 &32   &3.470  &3.252  &3.210   &3.221\\
   77  &
 $^\ddag$Y 4338    &dM4.5e    &18 &46 &44.1 &-23  &53 &32   &6.297  &5.680  &5.416   &5.486\\
   78  & BS 7120    &K3II      &18 &52 &05.8 &-22  &44 &08   &2.739  &2.120  &2.033   &2.056\\
   79  &
 $^\ddag$GL 748    &dM4       &19 &09 &38.0 & 02  &48 &36   &7.105  &6.557  &6.319   &6.382\\
   80  & BS 7615    &K0III     &19 &54 &25.7 & 34  &56 &58   &2.199  &1.716  &1.640   &1.660\\
   81  &
 $^\ddag$BS 7773   &B9.5V     &20 &17 &53.5 &-12  &55 &04   &4.825  &4.859  &4.859   &4.859\\
   82  &
 $^\ddag$GL 811.1  &dM4       &20 &54 &04.0 &-10  &37 &36   &7.832  &7.185  &6.946   &7.009\\
   83  &
 $^\ddag$HD201941  &A2        &21 &10 &13.6 & 02  &26 &12   &6.696  &6.657  &6.626   &6.634\\
   84  & BS 8143    &B9Iab     &21 &15 &27.0 & 39  &11 &04   &3.886  &3.838  &3.797   &3.808\\
   85  &
 $^\ddag$HD203856  &A0        &21 &21 &37.1 & 39  &48 &12   &6.926  &6.887  &6.861   &6.868\\
   86  & HD205772   &A3        &21 &35 &33.6 &-41  &16 &26   &7.775  &7.688  &7.657   &7.665\\
   87  & SAO34401   &F0        &22 &21 &47.7 & 54  &57 &12   &7.933  &7.766  &7.734   &7.742\\
   88  &
 $^\ddag$BS 8541   &B9Iab     &22 &22 &29.0 & 49  &13 &21   &4.305  &4.267  &4.235   &4.243\\
   89  & BS 8551    &K0III     &22 &25 &19.6 & 04  &26 &39   &2.956  &2.378  &2.312   &2.329\\
   90  &
 $^\ddag$Y 5546    &dM5       &22 &50 &36.2 &-14  &31 &34   &5.980  &5.344  &5.066   &5.140\\
       & 
     $^*$GL 299     &          &08-&09 &14.5 & 08  &56 &01   & 8.38  &7.915  &7.640   &7.713\\
\hline
\multicolumn{13}{l}{\extravspace
\llap{$^\dag$}{$K'=K+0.265*(H-K)$}
}\\
\multicolumn{13}{l}{
\llap{$^\ddag$}{multiple star system}
}\\
\multicolumn{13}{l}{
\llap{$^*$}{GL299 has a high proper motion (1163, -5079 mas/yr) and was thus dropped off the list,}
}\\
\multicolumn{13}{l}{
{but was previously available}
}
\end{tabular}
\end{center}
\end{sidewaystable}

%%\citep{1992AJ....103..332W}


==> tables/ex_ch3/table_UKIRT_FS.tex <==
% $Id: table_UKIRT_FS.tex,v 1.1 2001/04/16 01:56:11 jim Exp $
%
% Table of UKIRT Faint Standards from May of 1998
%
\begin{sidewaystable}
\caption{UKIRT Faint Standards - May 1998 \label{table_UKIRT_FS}}
\begin{center}
\begin{tabular}{|l|c|c|c|r|r|r|r|c|r|c|r|c|}
\hline\extravspace
     &\multicolumn{3}{c}{R.A. (J1950.0)} &\multicolumn{3}{c|}{Dec. (J1950.0)} &&&&&&\\
Name & h & m & s & \arcdeg & \arcmin & \arcsec & $K$ & $K$ $\sigma$ &
 $J-K$ & $J-K$ $\sigma$ & $H-K$ & $H-K$ $\sigma$ \\
\hline\extravspace
%Name       &h        &m        &s          &deg       &m        &s        &$K$          &$K$ err     &$J-K$        &$J-K$ err   &$H-K$        &$H-K$ err\\
FS01       &00       &31       &22.7       &-12       &24       &29       &12.967       &0.021       & 0.462       &0.011       & 0.081       &0.012\\
FS02       &00       &52       &36.0       &+00       &26       &58       &10.466       &0.003       & 0.247       &0.003       & 0.038       &0.003\\
FS03       &01       &01       &46.6       &+03       &57       &34       &12.822       &0.007       &-0.222       &0.011       &-0.097       &0.007\\
FS04       &01       &52       &03.7       &+00       &28       &20       &10.264       &0.005       & 0.292       &0.003       & 0.040       &0.007\\
FS05       &01       &52       &04.7       &-07       &00       &47       &12.342       &0.006       &-0.007       &0.004       &-0.002       &0.004\\
FS06       &02       &27       &39.2       &+05       &02       &34       &13.374       &0.015       &-0.135       &0.014       &-0.069       &0.012\\
FS07       &02       &54       &47.2       &+00       &06       &39       &10.940       &0.005       & 0.165       &0.012       & 0.037       &0.010\\
FS08       &02       &55       &12.9       &+00       &04       &04       & 8.313       &0.006       & 0.766       &0.002       & 0.129       &0.004\\
FS09       &02       &55       &38.8       &+00       &58       &54       & 8.266       &0.006       & 0.884       &0.003       & 0.158       &0.005\\
FS10       &03       &46       &17.4       &-01       &07       &38       &14.919       &0.072       &-0.170       &0.077       &-0.049       &0.060\\
FS11       &04       &50       &25.4       &-00       &19       &34       &11.278       &0.018       & 0.076       &0.025       & 0.016       &0.019\\
FS12       &05       &49       &34.8       &+15       &52       &37       &13.898       &0.003       &-0.217       &0.014       &-0.091       &0.018\\
FS13       &05       &54       &33.8       &+00       &00       &53       &10.135       &0.003       & 0.382       &0.002       & 0.047       &0.005\\
FS14       &07       &21       &41.2       &-00       &27       &10       &14.261       &0.012       &-0.153       &0.005       &-0.079       &0.020\\
FS15       &08       &48       &21.9       &+11       &55       &02       &12.360       &0.021       & 0.418       &0.008       & 0.060       &0.007\\
FS16       &08       &48       &31.0       &+12       &00       &36       &12.631       &0.008       & 0.340       &0.006       & 0.038       &0.005\\
\hline
\multicolumn{13}{|r|}{\extravspace\it continued on the next page}\\
\hline
\end{tabular}
\end{center}
\begin{quote}
  The UKIRT Faint Standards as published on the UKIRT website in May
  of 1998. These were the values used in this dissertation.  Some of
  the stars on this list were removed since that time, and some
  magnitudes may have changed. In addition, the errors in measurements
  are different-generally, better measurements are available. At the
  time of this dissertation, the standards had yet to be formally
  published.  Coordinate epoch is J1950.0.
\end{quote}
\end{sidewaystable}

\begin{sidewaystable}
\begin{center}
Table~\ref{table_UKIRT_FS}, continued.\hfill\\[2ex]
\begin{tabular}{|l|c|c|c|r|r|r|r|c|r|c|r|c|}
\hline\extravspace
     &\multicolumn{3}{c}{R.A. (J1950.0)} &\multicolumn{3}{c|}{Dec. (J1950.0)} &&&&&&\\
Name & h & m & s & \arcdeg & \arcmin & \arcsec & $K$ & $K$ $\sigma$ &
 $J-K$ & $J-K$ $\sigma$ & $H-K$ & $H-K$ $\sigma$ \\
\hline\extravspace
FS17       &08       &48       &35.4       &+12       &03       &26       &12.270       &0.007       & 0.411       &0.007       & 0.073       &0.003\\
FS18*      &08       &51       &02.1       &-00       &25       &14       &10.522       &0.008       & 0.292       &0.003       & 0.031       &0.003\\
FS19       &10       &31       &14.5       &-11       &26       &08       &13.796       &0.025       &-0.231       &0.021       &-0.142       &0.047\\
FS20       &11       &05       &27.6       &-04       &53       &04       &13.473       &0.017       &-0.120       &0.015       &-0.069       &0.012\\
FS21       &11       &34       &27.6       &+30       &04       &35       &13.132       &0.004       &-0.184       &0.033       &-0.101       &0.037\\
FS23       &13       &39       &25.7       &+28       &44       &59       &12.374       &0.000       & 0.623       &0.004       & 0.072       &0.018\\
FS24       &14       &37       &33.3       &+00       &14       &36       &10.753       &0.008       & 0.151       &0.006       & 0.019       &0.004\\
FS25       &15       &35       &59.9       &+00       &24       &03       & 9.756       &0.017       & 0.475       &0.003       & 0.070       &0.005\\
FS26       &16       &34       &26.3       &-00       &28       &39       & 7.972       &0.009       & 0.858       &0.004       & 0.155       &0.006\\
FS27       &16       &38       &54.2       &+36       &26       &56       &13.123       &0.018       & 0.371       &0.013       & 0.058       &0.014\\
FS28*      &17       &41       &32.5       &-00       &23       &44       &10.597       &0.016       & 0.148       &0.010       & 0.047       &0.005\\
FS29       &21       &49       &53.0       &+02       &09       &16       &13.346       &0.024       &-0.171       &0.011       &-0.075       &0.012\\
FS30       &22       &39       &11.3       &+00       &56       &55       &12.015       &0.020       &-0.092       &0.013       &-0.036       &0.005\\
FS31       &23       &09       &50.4       &+10       &30       &46       &14.039       &0.010       &-0.241       &0.020       &-0.120       &0.017\\
FS32       &23       &13       &38.2       &-02       &06       &58       &13.664       &0.012       &-0.205       &0.011       &-0.088       &0.015\\
FS33       &12       &54       &35.1       &+22       &18       &08       &14.240       &0.016       &-0.223       &0.010       &-0.078       &0.024\\
FS34       &20       &39       &41.9       &-20       &15       &21       &12.989       &0.011       &-0.170       &0.008       &-0.070       &0.009\\
FS35       &18       &24       &44.5       &+04       &01       &17       &11.757       &0.017       & 0.474       &0.008       & 0.089       &0.005\\
\hline
\multicolumn{13}{l}{\extravspace
Coordinate epoch is J1950.0. Stars marked with (*) are
double.
}
\end{tabular}
\end{center}
\end{sidewaystable}


==> tables/ex_ch3/table_UKIRT_FS_KJ.tex <==
% $Id: table_UKIRT_FS_KJ.tex,v 1.1 2001/04/16 01:56:11 jim Exp $
%
% Table of Derived J,H,K, K' mags from UKIRT Faint Standards from May of 1998
%

\begin{table}
\caption{Derived UKIRT Faint Standards Magnitudes - May 1998
   \label{table_UKIRT_FS_KJ}}
\vspace{4ex}
\begin{center}
\small
\begin{tabular}{|l|r|c|r|c|r|c|r|c|}
\hline\extravspace
Name &$J$ &$J$ $\sigma$ &$H$ &$H$ $\sigma$ &$K$ &$K$ $\sigma$ &$K^{\prime}$ &$K^{\prime}$ $\sigma$ \\
\hline\extravspace
%Name         J        J err     H       H err     K       K err     K'      K' err
FS01          &13.429  &0.024   &13.048  &0.084   &12.967  &0.021   &12.988  &0.021\\
FS02          &10.713  &0.004   &10.504  &0.038   &10.466  &0.003   &10.476  &0.003\\
FS03          &12.600  &0.013   &12.725  &0.097   &12.822  &0.007   &12.796  &0.007\\
FS04          &10.556  &0.006   &10.304  &0.040   &10.264  &0.005   &10.275  &0.005\\
FS05          &12.335  &0.007   &12.340  &0.006   &12.342  &0.006   &12.341  &0.006\\
FS06          &13.239  &0.021   &13.305  &0.071   &13.374  &0.015   &13.356  &0.015\\
FS07          &11.105  &0.013   &10.977  &0.037   &10.940  &0.005   &10.950  &0.006\\
FS08         & 9.079   &0.006  & 8.442   &0.129  & 8.313   &0.006  & 8.347   &0.006\\
FS09         & 9.150   &0.007  & 8.424   &0.158  & 8.266   &0.006  & 8.308   &0.006\\
FS10          &14.749  &0.105   &14.870  &0.087   &14.919  &0.072   &14.906  &0.074\\
FS11          &11.354  &0.031   &11.294  &0.024   &11.278  &0.018   &11.282  &0.019\\
FS12          &13.681  &0.014   &13.807  &0.091   &13.898  &0.003   &13.874  &0.006\\
FS13          &10.517  &0.004   &10.182  &0.047   &10.135  &0.003   &10.147  &0.003\\
FS14          &14.108  &0.013   &14.182  &0.080   &14.261  &0.012   &14.240  &0.013\\
FS15          &12.778  &0.022   &12.420  &0.064   &12.360  &0.021   &12.376  &0.021\\
FS16          &12.971  &0.010   &12.669  &0.039   &12.631  &0.008   &12.641  &0.008\\
FS17          &12.681  &0.010   &12.343  &0.073   &12.270  &0.007   &12.289  &0.007\\
FS18*         &10.814  &0.009   &10.553  &0.032   &10.522  &0.008   &10.530  &0.008\\
FS19          &13.565  &0.033   &13.654  &0.144   &13.796  &0.025   &13.758  &0.028\\
FS20          &13.353  &0.023   &13.404  &0.071   &13.473  &0.017   &13.455  &0.017\\
FS21          &12.948  &0.033   &13.031  &0.101   &13.132  &0.004   &13.105  &0.011\\
FS23          &12.997  &0.004   &12.446  &0.072   &12.374  &0.000   &12.393  &0.005\\
FS24          &10.904  &0.010   &10.772  &0.021   &10.753  &0.008   &10.758  &0.008\\
FS25          &10.231  &0.017  & 9.826   &0.072  & 9.756   &0.017  & 9.775   &0.017\\
FS26         & 8.830   &0.010  & 8.127   &0.155  & 7.972   &0.009  & 8.013   &0.009\\
FS27          &13.494  &0.022   &13.181  &0.061   &13.123  &0.018   &13.138  &0.018\\
FS28*         &10.745  &0.019   &10.644  &0.050   &10.597  &0.016   &10.609  &0.016\\
FS29          &13.175  &0.026   &13.271  &0.079   &13.346  &0.024   &13.326  &0.024\\
FS30          &11.923  &0.024   &11.979  &0.041   &12.015  &0.020   &12.005  &0.020\\
FS31          &13.798  &0.022   &13.919  &0.120   &14.039  &0.010   &14.007  &0.011\\
FS32          &13.459  &0.016   &13.576  &0.089   &13.664  &0.012   &13.641  &0.013\\
FS33          &14.017  &0.019   &14.162  &0.080   &14.240  &0.016   &14.219  &0.017\\
FS34          &12.819  &0.014   &12.919  &0.071   &12.989  &0.011   &12.970  &0.011\\
FS35          &12.231  &0.019   &11.846  &0.091   &11.757  &0.017   &11.781  &0.017\\
\hline
\end{tabular}
\begin{quote}
  Coordinate epoch is J1950.0. $K^{\prime} = K + 0.265(H-K)$ (from
  Wainscoat and Cowie (1992)).  Errors are quadratic sum 1 $\sigma$
  values for $J$,$H$,$K^{\prime}$.  Stars marked with (*) are double.
\end{quote}
\end{center}
\end{table}

